Towards Practical Robustness Analysis for DNNs based on PAC-Model Learning

To analyse local robustness properties of deep neural networks (DNNs), we present a practical framework from a model learning perspective. Based on black-box model learning with scenario optimisation, we abstract the local behaviour of a DNN via an affine model with the probably approximately correct (PAC) guarantee. From the learned model, we can infer the corresponding PAC-model robustness property. The innovation of our work is the integration of model learning into PAC robustness analysis: that is, we construct a PAC guarantee on the model level instead of sample distribution, which induces a more faithful and accurate robustness evaluation. This is in contrast to existing statistical methods without model learning. We implement our method in a prototypical tool named DeepPAC. As a black-box method, DeepPAC is scalable and efficient, especially when DNNs have complex structures or high-dimensional inputs. We extensively evaluate DeepPAC, with 4 baselines (using formal verification, statistical methods, testing and adversarial attack) and 20 DNN models across 3 datasets, including MNIST, CIFAR-10, and ImageNet. It is shown that DeepPAC outperforms the state-of-the-art statistical method PROVERO, and it achieves more practical robustness analysis than the formal verification tool ERAN. Also, its results are consistent with existing DNN testing work like DeepGini.

==> CCproof.tex <==
\newpage
\appendix
\section{CC's Proof}
Without loss of generality,
let $L$ be a local Lipschitz constant of the DNN,
i.e. 
\[
||\bm{\Delta}(\x)-\bm{\Delta}(\x')||_\infty \le L ||\x - \x'||_\infty
\]
for any $\x,\x'\in B(\hat\x,r)$.
Let 
\[
\delta = \max\limits_{\substack{j=1,\ldots,n \\ \x\in B(\hat\x,r)}} \widetilde{\Delta}_j(\x)+\lambda.
\]
Denote by $H^d(\cdot)$ the $d$-dimensional Hausdorff measure.
We use the symbol ``$\oplus$'' as the concatenation operator of a vector and a number.
Consider the vector space $\mathbb{R}^{m+1}$ and a certain $\Delta = \Delta_j$. 
For $\Delta=a_0+a_1x_1+\cdots+a_m$, 
define the reflection $R$ w.r.t.
the hyperplane.
Denote by $\Delta_R$ and $\widetilde{\Delta}_R$
the images of $\Delta$ and $\widetilde{\Delta}$.
For simplicity,
here we reuse $a_i$ to denote the coefficients of $\widetilde{\Delta}_R$.
Then, we have every $a_i$ is positive. 
Furthermore, for the region $B(R(\hat x),r)$,
the local Lipschitz constant
$L$ and maximum value $\delta$ still hold
for $\Delta_R$ and $\widetilde{\Delta}$, respectively. 
Meanwhile, we also have
\[
\mathbb{P}(\Delta_R(\x) > \widetilde{\Delta}_R(\x)+\lambda) < \epsilon.
\]
Let
\[
S=\{ \x \oplus 0 \in \mathbb{R}^{m+1} | \Delta_R(\x) \ge 0\},
\]
and
\[
\begin{aligned}
Z=\{ \x \oplus y\in \mathbb{R}^{m+1}  | \Delta_R(\x) \ge \widetilde{\Delta}_R(\x)+\lambda,
 y= \widetilde{\Delta}_R(\x) \}.
\end{aligned}
\]
Assume there is a central projection $P$ from a certain point $\dot{\x} \oplus \dot{y}$ onto the hyperplane $\widetilde{\Delta}_R(\x)+\lambda-y=0$.
Let 
\[
\dot{x}_i = 
  \max\limits_{\x \oplus \, 0\in S} {x_i}. 
\]
% \[
% \dot{x}_i = \left\{
% \begin{array}{ll}
%   \max\limits_{\x \oplus \, 0\in S} {x_i}   & a_i > 0, \\
%   \min\limits_{\x \oplus \, 0\in S} {x_i}   & a_i < 0.
% \end{array}
% \right.
% \]

Denote by $S'$ the set of the images
of all elements in $S$ by the projection $P$.
Then, there exist a certain point $\dot{\x} \oplus \dot{y}$ with
$\dot{\x}\in B(R(\hat\x),r)$ and $\dot{y}\le 2rL$ such that $S'\subseteq Z$.

\begin{figure}[h]
    \centering
        \centering
        \includegraphics[width=0.8\linewidth]{fig_c.eps}
    \caption{projection}
    \label{fig:c}
\end{figure}

For $\x\oplus y\in S$ and its image $\x' \oplus y' \in S'$, we have
\[
\begin{aligned}
& x'_i = \dot{x}_i + t(x_i-\dot{x}_i) \quad \text{for $i=1,\ldots,m$},\\
& y' = \dot{y}+t(0-\dot{y}),\\
& a_0+a_1x'_1+\cdots+a_mx'_m + \lambda - y'=0.
\end{aligned}
\]
Then,
\[
x_i = \frac{1}{t} x'_i + (1-\tfrac{1}{t}) \dot{x_i},
\]
and
\[
t=-\frac{a_0}{\dot{y}}-\frac{a_1}{\dot{y}}x'_1-\cdots-\frac{a_m}{\dot{y}}x'_m-\frac{\lambda}{\dot{y}}+1.
\]
We compute
\[
\begin{aligned}
\frac{\partial x_i}{\partial x'_i} & =  \frac{1}{t}-\frac{1}{t^2} \frac{\partial t}{\partial x'_i} x'_i 
+ \frac{1}{t^2}\frac{\partial t}{\partial x'_i}\dot{x}_i\\
& = \frac{1}{t}(1 + \frac{1}{t}\frac{\partial t}{\partial x'_i}(\dot{x}_i-x'_i)),
\end{aligned}
\]
and for $k\neq i$,
\[
\begin{aligned}
\frac{\partial x_i}{\partial x'_k} & =  -\frac{1}{t^2} \frac{\partial t}{\partial x'_k} x'_i
+ \frac{1}{t^2}\frac{\partial t}{\partial x'_k}\dot{x}_i\\
& = \frac{1}{t^2}(\frac{\partial t}{\partial x'_k}(\dot{x}_i-x'_i)).
\end{aligned}
\]
By $\frac{\partial t}
{\partial x'_j}=-\frac{a_j}{\dot{y}}$ and $\frac{1}{t}=\frac{\dot{y}}{\dot{y}-y'}$, 
we have
\[
d x_i =
\frac{\dot{y}}{\dot{y}-y'}\left(1- \frac{\dot{x}_i-x'_i}{\dot{y}-y'}
\sum_j (a_j d x'_j)\right)
\]
% \[
% \frac{\partial x_i}{\partial x'_i} =
% \frac{\dot{y}}{\dot{y}-y'}(1- \frac{\dot{x}_i-x'_i}{\dot{y}-y'}a_i),
% \]
% and
% \[
% \frac{\partial x_i}{\partial x'_k} =
% \frac{\dot{y}}{\dot{y}-y'}(- \frac{\dot{x}_i-x'_i}{\dot{y}-y'}a_k).
% \]
Thus,
\[
d x_i\le
\frac{2rL}{2rL-\delta}(1- \frac{a_i}{L})dx'_i.
\]
Therefore, we have
\[
\begin{aligned}
& H^m(\cup_{j=1}^n S_j) 
= \iint \cdots \int _{\cup_{j=1}^n S_j} dx_1 dx_2\cdots dx_m\\
& \le (\frac{2rL}{2rL-\delta})^m \prod_{i=1}^m (1- \frac{\min_j a_{ji} }{L})  \iint \cdots \int _{\cup_{j=1}^n S'_j} dx'_1 dx'_2\cdots dx'_m\\
& \le  (\frac{2rL}{2rL-\delta})^m \prod_{i=1}^m (1- \frac{\min_j a_{ji} }{L}) H^m(Z'_j),
\end{aligned}
\]
where $a_ji$ denotes the coefficient
of $x_i$ for $\widetilde{\Delta}_R$,
and $Z'_j=\{(x_1,\ldots,x_m)\in\mathbb{R}^m | (x_1,\ldots,x_m,y) \in  Z_j \}$.
Finally, by the inverse of the reflection,
we immediately have
\[
\mathbb{P}(\bm{\Delta}(\x)\ge 0 ) \le (\frac{2rL}{2rL-\delta})^m \prod_{i=1}^m (1- \frac{\min_j|a_{ji}|}{L}) \epsilon.
\]



==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> old-experiments.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%   
% \section{Experiments} \label{sec:experiment}
% We implement our approach as a prototype called DeepPAC. The implementation is based on Python 3.7.8. We use CVXPY~\cite{diamond2016cvxpy} as the modeling language for linear programming and GUROBI~\cite{gurobi} as the LP solver. All experiments are conducted on a Windows 10  PC with Intel i7 8700, GTX 1660Ti, and 16G RAM.
% %\paragraph{Datasets.}
% %The MNIST~\cite{L1998Gradient} database contains greyscale pictures of handwritten numbers with $60\,000$ images for training and $10\,000$ for testing. The image size of the MNIST database is $28\times28$. The CIFAR-10~\cite{cifar10} dataset contains color images in ten classes. Every class has $5\,000$ images for training and $1\,000$ images for testing. The image size of the CIFAR-10 dataset is $32\times32$. Both datasets are used in image classification. Before training, we normalized both the MNIST dataset and the CIFAR-10 dataset and performed random cropping and horizontal flipping during CIFAR-10 training.

% We choose MNIST~\cite{L1998Gradient} and CIFAR-10~\cite{cifar10} as the datasets.
% On MNIST, we trained six fully connected networks (FNN1--6) with the structures of varying numbers of hidden layers and hidden neurons in each layer:
% $3\times50$, $3\times100$, $3\times200$, $6\times200$, $9\times200$, and $6\times500$.
% For the CIFAR-10 dataset, we trained a large convolutional neural network~\cite{vgg} (VGG16) and four residual neural networks~\cite{resnet} (ResNet18, ResNet50, ResNet101, ResNet152). The number of parameters are $14.7$M, $11.2$M, $23.5$M, $42.5$M and $58.2$M respectively. 
% %To train the DNNs, we used the stochastic gradient descent optimizer with learning rates $0.001$ (for MNIST) and $\{0.1, 0.01, 0.001\}$ (for CIFAR-10 with $200$ epochs of each rate).

% %The stochastic gradient descent optimizer is still used for training, using $0.1$, $0.01$, and $0.001$ as the learning rate successively, and each learning rate is trained for $200$ epochs.



% \subsection{Maximal PAC Robustness Radius} \label{subsec:verificationex}
% %For the verification task, 
% We pick the $0$th, $128$th, and $256$th images from the MNIST training set as the examples, and verify them with confidence $1-\eta=99.9\%$ and error rates of $\epsilon=0.05$, $0.01$, and $0.001$, respectively. We invoke our \emph{focused learning algorithm}, %and use binary search to find a relatively large robustness radius $r$ so that it is PAC robust, and a relatively small unsafe radius. 
% and use binary search to find the largest PAC robustness radius $r$ and the smallest unsafe radius. The main results are shown in Table~\ref{tab:mnist}.

% %It should be noted that because of the existence of probability, the binary search may not be stable, and the result is obtained by fixing the random seed. 




% \paragraph{Comparison with ERAN.}
% We compare our method with ERAN, using DeepPoly~\cite{deeppoly} to verify the DNNs and record the maximum robustness radius that can be verified. The maximum robustness radius is given in the practical sense (a grayscale value from $0$ to $255$). 
% %The corresponding results of the three error rates are shown in Table~\ref{tab:mnist}.
% ERAN is the state-of-the-art verification tool based on abstract interpretation. It is sound so
% its error rate is zero. 
% Therefore, it is conceivable that ERAN always has a smaller robustness radius than our method. 
% %Besides, the precision loss of the abstract interpretation method increases along with the depth of the neural network. 

% %For instance FNN6 and the 256th image, our PAC verified robustness radius is 5-times larger than the one guaranteed by ERAN. 
% % When using DeepPAC, the robustness radius obtained shows obvious differences on different networks. But for ERAN, it remains more or less the same. 
% % It is interesting to note that, the network FNN5 has larger robustness radii on the three images than the other networks.
% % From a quantitative perspective, the radius of PAC robustness computed by DeepPAC has relatively better practical meanings.

% An interesting observation is that
% the robustness radii of the FNNs verified by ERAN are quite close, but significantly different by DeepPAC.
% This is because ERAN and DeepPAC measure the local robustness from two different concepts, i.e. exact and probabilistic, respectively.
% Although ERAN is sound, from a quantitative perspective, the radius of PAC robustness computed by DeepPAC has relatively better practical meanings.
% For example, FNN5 is shown to be more robust than the other networks
% via the radii of PAC robustness on these three images.

% \paragraph{Comparison with the Sampling-based Method.} We also compare our method with the sampling-based method proposed in \cite{anderson2020certifying}. Note that the radii in the column ``$\times$'' in Table \ref{tab:mnist} are always larger than the exact robustness radii, since real counterexamples can be found by DeepPAC in the corresponding closed $L_{\infty}$ ball. Therefore, we conclude from Table \ref{tab:mnist} that the robustness radii given by the sampling-based method in \cite{anderson2020certifying} are much larger than the exact radii and thus too inaccurate. Furthermore, referring the radii in the column ``$\checkmark$'' computed by DeepPAC, we reach a conclusion that our method can give more precise evaluation on robustness radii and thus analyse local robustness of DNNs more practically than the sampling-based method in \cite{anderson2020certifying}.

% %unreasonably large for all the cases: they are much larger than the exact radii and the radii given by the sampling-based method in \cite{anderson2020certifying} are too inaccurate. %local robustness on these cases. 


% \begin{table*}[t]\footnotesize
% \centering
% \scalebox{0.9}{
% \begin{tabular}{|c|c|c|c|ccc|ccc|ccc|}
% \hline
% \multirow{2}{*}{Index} & \multirow{2}{*}{DNN} & \multirow{2}{*}{ERAN} & \multirow{2}{*}{Sampling} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.001$} \\
%  &  &  & & \checkmark & ? & $\times$ & \checkmark & ? & $\times$ & \checkmark & ? & $\times$ \\ \hline
% \multirow{6}{*}{0} & FNN~1 & 2 & 26 & 4 & 5 & 6 & 4 & 5 & 6 & 4 & 5 & 6 \\
%  & FNN~2 & 4 & 58 & 5 & 6 & 7 & 5 & 6 & 7 & 5 & 6 & 7 \\
%  & FNN~3 & 4 & 47 & 9 & -- & 10 & 9 & -- & 10 & 9 & -- & 10 \\
%  & FNN~4 & 4 & 37 & 11 & -- & 12 & 11 & -- & 12 & 11 & -- & 12 \\
%  & FNN~5 & 6 & 92 & 22 & -- & 23 & 22 & -- & 23 & 22 & -- & 23 \\
%  & FNN~6 & 3 & 37 & \enspace 10 \enspace & -- & \enspace 11 \enspace & \enspace 10 \enspace & -- & \enspace 11 \enspace &  \enspace 10 \enspace & -- & \enspace 11 \enspace \\ \hline
% \multirow{6}{*}{128} & FNN~1 & 4 & 59 & 7 & [8,9] & 10 & 7 & [8,9] & 10 & 7 & [8,9] & 10 \\
%  & FNN~2 & 7 & 148 & 23 & [24,31] & 32 & 23 & [24,31] & 32 & 23 & [24,30] & 31 \\
%  & FNN~3 & 6 & 101 & 27 & 28 & 29 & 26 & [27,28] & 29 & 26 & [27,28] & 29 \\
%  & FNN~4 & 4 & 79 & 21 & [22,24] & 25 & 21 & [22,24] & 25 & 21 & [22,24] & 25 \\
%  & FNN~5 & 5 & 112 & 50 & -- & 51 & 50 & -- & 51 & 51 & -- & 52 \\
%  & FNN~6 & 3 & 78 & 25 & -- & 26 & 25 & -- & 26 & 25 & -- & 26 \\ \hline
% \multirow{6}{*}{256} & FNN~1 & 4 & 46 & 9 & 10 & 11 & 9 & 10 & 11 & 9 & 10 & 11 \\
%  & FNN~2 & 5 & 45 & 12 & -- & 13 & 12 & -- & 13 & 12 & -- & 13 \\
%  & FNN~3 & 5 & 60 & 13 & -- & 14 & 13 & -- & 14 & 13 & -- & 14 \\
%  & FNN~4 & 3 & 51 & 16 & -- & 17 & 16 & -- & 17 & 16 & -- & 17 \\
%  & FNN~5 & 3 & 53 & 22 & -- & 23 & 21 & 22 & 23 & 21 & 22 & 23 \\
%  & FNN~6 & 3 & 47 & 15 & -- & 16 & 15 & -- & 16 & 15 & -- & 16 \\ \hline
% \end{tabular}
% }
% \caption{Verification results on MNIST. The column for ERAN provides the maximal robustness radius that DeepPoly can verify. The column for Sampling provides the maximal PAC robustness radius given by the sampling-based method in \cite{anderson2020certifying}, with error rate $\epsilon=0.001$ and confidence $1-\eta=99.9\%$. In the headline, ``$\checkmark$'' is the maximal PAC robustness radius we can check, ``$\times$'' offers the smallest radius such that DeepPAC can generate a counterexample, ``\,?\,'' indicates the unknown range of the radius, and ``\,--\,'' means that the item is empty.}
% \label{tab:mnist}
% \end{table*}

% \begin{table*}[!ht]
% \centering
% \scalebox{0.9}{
% \begin{tabular}{|c|ccc|ccc|ccc|c|}
% \hline
% \multirow{2}{*}{DNN} & \multicolumn{3}{c|}{Image 0} & \multicolumn{3}{c|}{Image 128} & \multicolumn{3}{c|}{Image 256} & \multirow{2}{*}{Avg Time} \\
%  & ~$r=1$~ & ~$r=2$~ & ~$r=3$~ & ~$r=1$~ & ~$r=2$~ & ~$r=3$~ & ~$r=1$~ & ~$r=2$~ & ~$r=3$~  & \\ \hline
% VGG16 & \checkmark & $\times$ & $\times$ & \checkmark & $\times$ & $\times$ & \checkmark & \checkmark & $\times$  & 120.05s \\
% ResNet18 & \checkmark & $\times$ & $\times$ & \checkmark & $\times$ & $\times$ & \checkmark & \checkmark & \checkmark   & 121.20s \\
% ResNet50 & \checkmark & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & \checkmark & ? & $\times$  & 140.65s \\
% ResNet101 & \checkmark & ? & $\times$ & $\times$ & $\times$ & $\times$ & \checkmark & \checkmark & ?  & 167.42s\\
% ~ResNet152~ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & \checkmark & ? & ?  &  182.90s\\ \hline
% \end{tabular}
% }
% \caption{CIFAR-10 verification result. With confidence $1-\eta=99.9\%$ and error rates of $\epsilon=0.01$, we verify the CIFAR-10 networks using radii 1, 2 and 3.
% %GPUPoly is supported by an Nvidia Tesla V100 GPU, while DeepPAC is supported by an GTX 1660Ti GPU.
% }
% \label{tab:CIFAR-10}
% \end{table*}




% \paragraph{Effect of Focused Learning.}
% %In our experiments, we have always invoked our \emph{focused learning optimization}.
% In the \emph{focused learning} optimization,
% we use the first batch of $K^{(1)}=2\,000$ random samples and the second batch of $K^{(2)}=8\,000$ random samples for the error rates $0.05$ and $0.01$,
% and use the first batch of $K^{(1)}=8\,000$ random samples and the second batch of $K^{(2)}=20\,000$ random samples for the error rate $0.001$.
% Overall, the running time is $140$, $90$, and $300$ seconds for these three error rates respectively. 
 
% %Through the experiment results, we can see that our method returns Unknown rarely. It shows that our method has learned the local behavior of the neural network, and the potential counterexamples generated are highly likely to be true counterexamples. 

% %It is interesting to observe that our method obtains similar results under different error rates. When we reduce the error rate from $0.05$ to $0.01$, most of the results agree, but we observe two cases where the PAC robustness radius decreases: they are FNN3 for the $128$th image and FNN5 for the $256$th image. As is illustrated by our running example (see Fig.~\ref{fig:netlearn}), a larger error rate may lead to a PAC claim, even when the original network is not robust.
% %As the error rate decreases, the radius becomes small in most cas.

% We observe that the maximum radius computed by our method is not sensitive to the error bound,
% because most of the results agree for error rate from $0.05$ to $0.01$. 
% One possible reason is that the affine template converges well under the training with a relatively small batch of samples, which implies that our method can learn a good approximation even at a relatively large error bound. This supports us to reduce the number of samples accordingly to extract the key features in the first phase.
% % \todo{good at high error,because linear function need fewer samples to converge}
% %The main reason is the parameter setting of our focused learning optimization: For a small error rate $\epsilon$, the bound $K$ is linear in $\frac{1}{\epsilon}$, but we reduce the number of samples in the first step to $K_1$ accordingly to extract key features first.
% %Thus, reducing error rate from $0.01$ to $0.001$ does not change the verified PAC radii and has also the same radii in counterexample generations.


% \paragraph{Scalability of DeepPAC.}
% %On the CIFAR-10 dataset, we also trained 5 neural networks of very large size and verified them with our method. 
% %It can be seen from Table~\ref{tab:CIFAR-10} that our method is still effective on larger datasets and networks.
% By using DeepPAC, we have also verified the PAC robustness of large-scale neural networks (VGG and ResNets) on the CIFAR-10 dataset.
% The results is shown in Table~\ref{tab:CIFAR-10}.
% GPUPoly~\cite{deeppolygpu} in the tool ERAN is a GPU accelerated version of DeepPoly, which is one of the state-of-the-art verifiers based on abstract interpretation.
% GPUPoly can verify a ResNet18 network in  $1\,021$ seconds on average with an Nvidia Tesla V100 GPU support, while DeepPAC can analyse a ResNet18 network in $121$ seconds using a PC with the limited resources.
% Note that DeepPAC is a black-box approach. What it utilizes is not the concrete internal structure of the neural network, but the pairs of input and output.
% Thus, compared with tools for white-box verification like ERAN, 
% % based on sound methods such as SMT and abstract interpretation, 
% our method has better efficiency and scalability in verifying the PAC robustness of large-scale neural networks.


% %. While these tools are white box approaches, ours is a black-box approach. We only care about the relationship between input and output, the internal structure of the network has almost no effect on efficiency. 

% %Thus, DeepPAC can verify networks much larger than previous methods.


% %Compared with previous tools based on SMT solvers and abstract interpretations, our method has better scalability. While these tools are white box approaches, ours is a black-box approach. We only care about the relationship between input and output, the internal structure of the network has almost no effect on efficiency. Thus, DeepPAC can verify networks much larger than previous methods.



% %The  tool ERAN supports GPUPoly~\cite{deeppolygpu}, DeepPoly running on GPUs. GPUPoly can verify a ResNet18 network in an average time of $1\,021$ seconds with an Nvidia Tesla V100 GPU support, while DeepPAC can analyze a ResNet18 network in $120$ seconds using a PC with Intel i7 8700, GTX 1660Ti, and 16G RAM. Our framework scales, as it can  handle  larger networks such as the ResNet152 network within three minutes.


% % \todo{1.Compare to DeepPoly,why larger? We can compare robustness of different nets, deeppoly cant always do that. 2. Very few unknown, our method is kind of sensitive. Fake counterexample very few. Relu Network can be seen as piecewise linear functions.\\ 3. Why different error rate comes with similar results? Focused Learning works. Linear model converge very well. $\lambda$ matters.}


% \subsection{Counterexample Generation}
% In this section, we report experiments of  counterexamples generation using DeepPAC.  %If the attack class score of the potential counterexample is higher than the correct class, it can be determined that a true counterexample is generated. 
% Our experiment generates counterexamples under the corresponding radii based on the minimum unsafe radii given in Sect.~\ref{subsec:verificationex} (see the column ``$\times$'' in Table~\ref{tab:mnist}). 

% % \paragraph{Mask Image.} 
% % A counterexample can be considered as an input which is obtained by adding a mask to the original picture. 
% % A mask image for the MNIST dataset is a black-and-white image. Black pixels are negative to attack if the value on these pixels increases, and vice versa for white pixels. 
% %On CIFAR-10, a mask image is a color image, and each pixel can be seen as an RGB triple. In the counterexample, if the corresponding channel value increases, the channel in the mask is set to $255$, or otherwise $0$. For example, when the red and green channels of a pixel increases, and the blue channel decreases, then the triple of the pixel is $(255, 255, 0)$, and the color is thus yellow. 


% % \begin{figure}[t]
% %     \centering
% %         \centering
% %         \includegraphics[width=0.8\linewidth]{fig_counter_mnist.eps}
% %     \caption{Counterexamples of neural networks for MNIST. We use the $0$th image as the original image. The radii are $6$, $7$, $10$, $12$, $23$, and $11$. The OLS (original label score w.r.t. ``5'') and ALS (attacking label score w.r.t. ``3'') are given below.}
% %     \label{fig:netcountermnist}
% % \end{figure}



% %\paragraph{MNIST Counterexamples for the networks FNN1--FNN6.}
% %\paragraph{Counterexamples.}
%  We choose the {$0$th} image of MNIST as an example, representing the number ``5''. %shown in Fig.~\ref{fig:netcountermnist}. 
%  For FNN1--FNN6, we use radii $6$, $7$, $10$, $12$, $23$, and $11$ (see column ``$\times$'' for $\epsilon=0.01$ of Table~\ref{tab:mnist}). We use the output corresponding to the number ``3'' to attack it. 
% The part A of Fig.~\ref{fig:netcountermnist_comb} shows the counterexamples and masks.
% The mask image here is a black-and-white image, in which black pixels are negative to attack when their values increase, and vice versa for white pixels. 


%  %of the corresponding radius of different networks on the original picture depicted above. 
%  % We measure the score difference as a quality of the counterexample: the score difference should tend to zero when it is closer to the decision boundary. We observe that the difference is below $1$ for five of them, and it is $2.7$ for FNN4.

% \iffalse
% % \begin{figure}[t]
% %     \centering
% %         \centering
% %         \includegraphics[width=0.8\linewidth]{fig_counter_cifar.eps}
% %     \caption{Counterexamples of neural networks for CIFAR-10. We use the $128$th image as the original image. The radii are $2$, $1$, $1$, $1$, and $2$, respectively. OLS means the original label score w.r.t. the class dog and ALS means the attacking label score w.r.t. the class cat.}
% %     \label{fig:netcountercifar}
% % \end{figure}

% % \paragraph{CIFAR-10 Counterexamples for VGG16 and ResNets.}
% % Similarly, we have performed experiments on the CIFAR-10 dataset. The original picture is the 128th image depicting a dog. Setting $\epsilon=0.01$, we use radius 2 for VGG16 and ResNet18, and radius 1 for other networks (see the column for Image 128 of Table~\ref{tab:CIFAR-10}). We use the output corresponding to the cat to attack it.
% % The results are given in Fig.~\ref{fig:netcountercifar}, which  shows that almost all networks have poor robustness, as  counterexamples can be generated with relatively small radii.
% % Moreover, the difference between the OLS and ALS is rather large: it is more than $6$ for all counterexamples, and is more than ten times larger for the VGG16.
% \fi

% % \lz{cifar: no picture for the case of focused area?}
% \begin{figure}[t]
%     \centering
%         \centering
%         \includegraphics[width=0.7\linewidth]{fig_counter_mnist_comb_2.eps}
%     \caption{Counterexamples of FNNs. We use the $0$th image of MNIST as the example. The radii are $6$, $7$, $10$, $12$, $23$, and $11$. The OLS (original label score w.r.t. ``5''), ALS (attacking label score w.r.t. ``3'') and \#CP (number of pixels changed) are given below.}
%     \label{fig:netcountermnist_comb}
% \end{figure}

% \paragraph{Counterexamples Using Important Pixels.}

% %We recall that focused learning optimization allows us to concentrate on those pixels with larger absolute values. In our conterexample generation scheme (see Sect.~\ref{sec:generation}), within the allowed radius, we take the image whose distance is the largest from the input in every pixel. 



% Furthermore, inspired by the focused learning optimization, we see that some pixels may have little effect on the attack. 
% %Thus, we now investigate properties of counterexamples when restricting to the set of pixels contributing most. 
% Thus, by ordering the importance of pixels, we give a variant method of counterexample generation with changing the least number of pixels.
% % \begin{figure}[t]
% %     \centering
% %         \centering
% %         \includegraphics[width=0.8\linewidth]{fig_counter_mnist_least.eps}
% %     \caption{Counterexamples of neural networks for MNIST with least important pixels changed. The \#CP (number of pixels changed) is given below the ALS.}
% %     \label{fig:netcountermnistleast}
% % \end{figure}
% For attack label $i$,
% we measure the importance of the pixel $x_j$ by the potential maximum increment which can be provided to $\widetilde\Delta_i(\x)$.
% Specifically, it is explicit as $\max({c}_{i,j}\cdot\min(255-x_j,r),-{c}_{i,j} \cdot \min(x_j,r))$, because $x_j$ can be changed in the range $[x_j-r,x_j+r]\cap[0,255]$.
% %Assume that we use the output $i$ to attack our image, and we have $\widetilde\Delta_i(\x) = c_{i,0}+\sum_{j} c_{i,j} x_j$. For pixel $x_j$, its contribution to the attack is approximately $|c_{i,j} r|$. The precise score of the pixel should take account of the fact that  pixel value has minimum $0$ and maximum $255$, so the precise score can be given by $Score(x_j)=\max({c}_{i,j}\cdot\min(255-x_j,r),-{c}_{i,j} \cdot \min(x_j,r))$. Our strategy is to determine the smallest number of pixels to change based on the contribution of each pixel. 
% The result is shown in the part B of Fig.~\ref{fig:netcountermnist_comb}.
% %among which black and white are similar to those in Fig.~\ref{fig:netcountermnist}, 
% Gray has been added to the colors of the mask to indicate the pixels unchanged. 
% % and gray pixels mean that corresponding pixels in the counterexample remain unchanged.
% %Experiment results are given in Fig.~\ref{fig:netcountermnistleast}. 
% % For networks from FNN1 to FNN6,  we only need to modify 56.9\%, 36.6\%, 42.9\%, 33.4\%, 32.0\%, and 46.4\%, respectively, of the most important pixels for attacking, 
% %from the original pictures. 
% %The successfully generated counterexamples confirm that some pixels have little effect on the attack.
% % which corroborates that the fact that some pixels have little effect on the attack.
% %At the same time, 
% %the mask image is more recognizable. It can be observed that the counterexample darkens the pixel regarding the true value and adds disturbance to the surroundings. 
% % we achieve very 
% The counterexamples are generated effectively
% with smaller score differences. %for the counterexamples,
% % which are at most $0.02$ in these cases. 
% Namely, the counterexample generated in this way is very close to the decision boundary.

% % \todo{1.MNIST counterexamples with scores \\ 3. CIFAR-10 counterexamples with scores \\ 2. counterexamples under different perturbations.}




% \paragraph{Comparison with Attacking Methods}
% %We also compare our counterexamples with those generated by attacking methods.
% The quality of a counterexample can be measured by the distance from its original image.
% We compare the minimum $L_\infty$ distance of our counterexamples with those generated by the white-box attack methods FGSM~\cite{fgsm}, DeepFool~\cite{DBLP:conf/cvpr/Moosavi-Dezfooli16}, and PGD~\cite{pgd}, and the black-box attack method GenAttack~\cite{GenAttack}. Our implementation is based on Foolbox~\cite{foolbox,foolboxnative}. The results are shown in Fig.~\ref{fig:attackcomparison}.
% As a black-box method, our tool outperforms the GenAttack on $16$ cases out of $18$ on MNIST, and $10$ out of $18$ on CIFAR-10.
% %Our score-based methods could even defeat these attacks in some cases.
% For the white-box methods, PGD is among the best on all benchmarks, followed by DeepFool. Notably, our method performs equally or better than its white-box counterparts (PGD, FGSM, and DeepFool) on $8$, $12$, and $9$ cases out of $18$ on MNIST and $4$, $11$, and $7$ out of $18$ on CIFAR-10, respectively.
% It is interesting to observe that our method even generates a better counterexample with smaller $L_\infty$ distance than PGD for FNN2 on the 256th image of MNIST.
% These results show that our method is competitive to these state-of-the-art attacking methods.


% %The recently proposed Hop-Skip-Jump attack can be seen as an adversarial example refinement procedure since it moves along the decision boundary. Our methods could sometimes defeat the Hop-Skip-Jump attack without such refinement procedure.

% % Another important criterion for black-box attacks is the query amounts. Table.~\ref{} is the results limited to 4,000 queries. It is easy to see that our methods is more stable than GenAttack and Hop-Skip-Jump attack. Under the limitation of the queries, our method can find adversarial samples with relatively less disturbance.


% % \begin{table}[t]
% % \centering
% % \begin{tabular}{ |p{1.2cm}<{\centering}| p{3cm}<{\centering} | p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}|p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}|  }
% % \hline
% % \multirow{2}{*}{~ Index ~} & \multirow{2}{*}{~ Network ~} & \multicolumn{3}{c|}{White-box} & \multicolumn{3}{c|}{Black-box} \\
% %  &  & {~ PGD ~} & {~ FGSM ~} & {~ DF ~} & {~ LS ~} & {~ GA ~} & {~ Ours ~}  \\ \hline
% % \multirow{6}{*}{0} & FNN1 & 6 & 7 & 6 & 24 & 11 & 6  \\ % \cline{2-8}
% %  & FNN2 & 7 & 7 & 7 & 22 & 14 & 7  \\ % \cline{2-8}
% %  & FNN3 & 10 & 10 & 10 & 35 & 18 & 10  \\  % \cline{2-8}
% %  & FNN4 & 10 & 10 & 10 & 33 & 18 & 12 \\ % \cline{2-8}
% %  & FNN5 & 17 & 21 & 20 & - & 30 & 23 \\ % \cline{2-8}
% %  & FNN6 & 11 & 11 & 11 & 30 & 18 & 11 \\ \hline  % \cline{1-8}
% % \multirow{6}{*}{128} & FNN1 & 10 & 11 & 10 & 37 & 22 & 10 \\
% %  & FNN2 & 31 & 52 & 28 & - & 53 & 32 \\
% %  & FNN3 & 27 & 34 & 29 & - & 41 & 29 \\
% %  & FNN4 & 19 & 29 & 22 & - & 29 & 25 \\
% %  & FNN5 & 27 & 29 & 28 & - & 46 & 51 \\
% %  & FNN6 & 19 & 43 & 32 & - & 34 & 26 \\ \hline
% % \multirow{6}{*}{256} & FNN1 & 11 & 11 & 11 & 47 & 19 & 11 \\
% %  & FNN2 & 14 & 17 & 12 & - & 22 & 13 \\
% %  & FNN3 & 14 & 19 & 15 & - & 24 & 14 \\
% %  & FNN4 & 11 & 12 & 12 & 39 & 21 & 17 \\
% %  & FNN5 & 12 & 17 & 21 & - & 20 & 23 \\
% %  & FNN6 & 13 & 15 & 14 & 46 & 22 & 16 \\ \hline
% % \end{tabular}
% % \caption{Comparision with attacking methods. We list the minimum $L_\infty$ radii to find an adversarial example for both white-box and black-box methods. ``\,--\,'' means that the attack failed.}
% % \label{tab:attackcomparison}
% % \end{table}


% \begin{figure}[t]
%     \centering
%     \subfloat{%[Unsafe\label{fig:netcounterA}]{%
%     % \begin{subfigure}{.5\linewidth}
%         % \centering
%         \includegraphics[width=0.32\linewidth]{P0.eps}}
%         % \caption{Unsafe}
% %       \label{fig:netcounter}
%     % \end{subfigure}%
%     \hfill
%     \subfloat{%[Unknown\label{fig:netcounterB}]{%
%     % \begin{subfigure}{.5\linewidth}
%          \centering
%         \includegraphics[width=0.32\linewidth]{P1.eps}}
%         % \caption{Unknown}
%  %       \label{fig:result0.4}
%     % \end{subfigure}\hfill
%     \hfill
%     \subfloat{%[Unknown\label{fig:netcounterC}]{%
%     % \begin{subfigure}{.5\linewidth}
%         % \centering
%         \includegraphics[width=0.32\linewidth]{P2.eps}}
%         % \caption{Unknown}
%  %       \label{fig:result0.4}
%     % \end{subfigure}
    
%         \subfloat{%[Unsafe\label{fig:netcounterA}]{%
%     % \begin{subfigure}{.5\linewidth}
%         % \centering
%         \includegraphics[width=0.32\linewidth]{C0.eps}}
%         % \caption{Unsafe}
% %       \label{fig:netcounter}
%     % \end{subfigure}%
%     \hfill
%     \subfloat{%[Unknown\label{fig:netcounterB}]{%
%     % \begin{subfigure}{.5\linewidth}
%         % \centering
%         \includegraphics[width=0.32\linewidth]{C1.eps}}
%         % \caption{Unknown}
%  %       \label{fig:result0.4}
%     % \end{subfigure}\hfill
%     \hfill
%     \subfloat{%[Unknown\label{fig:netcounterC}]{%
%     % \begin{subfigure}{.5\linewidth}
%         % \centering
%         \includegraphics[width=0.32\linewidth]{C2.eps}}
%         % \caption{Unknown}
%  %       \label{fig:result0.4}
%     % \end{subfigure}
    
    
%      \subfloat{%
%     % \begin{subfigure}{.5\linewidth}
%         % \centering
%         \includegraphics[width=0.6\linewidth]{Pbars.eps}}
    
%     \caption{The minimum $L_\infty$ distance of the adversarial examples generated by the attacking methods.}
%   \label{fig:attackcomparison}
% \end{figure}


% % \begin{table}[h]
% % \centering
% % \begin{tabular}{|c|c|ccc|ccc|ccc|}
% % \hline
% % \multirow{2}{*}{~ Index ~} & \multirow{2}{*}{~ Network ~} & \multicolumn{3}{c|}{Gradient} & \multicolumn{3}{c|}{Score} & \multicolumn{3}{c|}{Decision} \\
% %  &  & {~ PGD ~} & {~ FGSM ~} & {~ DF ~} & {~ LS ~} & {~ GA ~} & {~ Ours ~} & {~ Blend ~} & {~ Samp ~} & {~ HSJ ~} \\ \hline
% % \multirow{6}{*}{0} & FNN1 & 6 & 7 & 6 & 28 & 11 & 6 & 49 & 32 & 7 \\
% %  & FNN2 & 7 & 7 & 7 & 23 & 14 & 7 & 109 & 48 & 7 \\
% %  & FNN3 & 10 & 10 & 10 & 33 & 18 & 10 & 99 & 60 & 11 \\
% %  & FNN4 & 10 & 10 & 10 & 34 & 18 & 12 & 58 & 51 & 11 \\
% %  & FNN5 & 17 & 21 & 20 & - & 30 & 23 & 206 & 92 & 19 \\
% %  & FNN6 & 11 & 11 & 11 & 37 & 18 & 11 & 58 & 50 & 11 \\ \hline
% % \multirow{6}{*}{128} & FNN1 & 10 & 11 & 10 & 26 & 22 & 10 & 97 & 68 & 12 \\
% %  & FNN2 & 31 & 52 & 28 & - & 53 & 32 & 209 & 171 & 32 \\
% %  & FNN3 & 27 & 34 & 29 & - & 41 & 29 & 192 & 131 & 27 \\
% %  & FNN4 & 19 & 29 & 22 & - & 29 & 25 & 125 & 93 & 20 \\
% %  & FNN5 & 27 & 29 & 28 & - & 46 & 51 & 184 & 146 & 32 \\
% %  & FNN6 & 19 & 43 & 32 & - & 34 & 26 & 112 & 96 & 22 \\ \hline
% % \multirow{6}{*}{256} & FNN1 & 11 & 11 & 11 & 43 & 19 & 11 & 80 & 61 & 12 \\
% %  & FNN2 & 14 & 17 & 12 & 37 & 22 & 13 & 70 & 59 & 14 \\
% %  & FNN3 & 14 & 19 & 15 & - & 24 & 14 & 102 & 78 & 18 \\
% %  & FNN4 & 11 & 12 & 12 & 34 & 21 & 17 & 82 & 64 & 12 \\
% %  & FNN5 & 12 & 17 & 21 & 28 & 20 & 23 & 86 & 64 & 13 \\
% %  & FNN6 & 13 & 15 & 14 & - & 22 & 16 & 72 & 59 & 16 \\ \hline
% % \end{tabular}
% % \caption{Comparision with attacking methods}
% % \label{tab:attackcomparison}
% % \end{table}

% \iffalse
% \section{Explanation of Attacking} \label{sec:explanation}
% In this section, we use our learned functions to give key features for both the classification and the attacking with a given label  as a local explanation. With the explanation, we can see which pixels make the most contribution to protecting the classification label from the attack and which tend to make the attack possible.

% The model we learn approximates the behaviour of the neural network in a local area surrounding $\hat{\bm x}$. We have chosen affine functions as templates, so the absolute value of the  synthesized coefficients indicate how much the corresponding pixel values affect the score difference. Recall this is also the essential idea exploited in our focused learning optimization.  
% %In this section, we  discuss how these key pixels can help explain our attacking model.
% The positive or negative of the coefficient indicates the direction of the influence of this input dimension on the neural network. What we learned is the score difference of the neural network, i.e. $\Delta_i(\x)=f_i(\x)-f_\ell(\x)$, where $i$ corresponds to the output label used to attack the network. Stated differently, we want to generate an input so that $f_i(\x)>f_\ell(\x)$.  We start from our approximating function $\widetilde\Delta_i(\bm x)=c_0+\sum_i c_i x_i$. The absolute value $|c_i|$ of the coefficient $c_i$ determines the influence of the current pixel on the classification result. Note that  $f_i(\x)$ can be approximated by $f_\ell(\x) + \widetilde \Delta_i(\x) =  f_\ell(\x) +c_0+ \sum_i c_i x_i$. Thus we have
% \begin{itemize}
% \item if $c_i>0$, increasing $x_i$ will enlarge the  value of $\widetilde \Delta_i(\x)$, which is beneficial to the attacking label, whereas
% \item if $c_i<0$, increasing $x_i$ will reduce the value of $\widetilde \Delta_i(\x)$, which  is beneficial to the classification label.
% \end{itemize}


% % The coefficient $\bm{c}_i$ of linear model $\widetilde\Delta(\bm{x})_i$ can be viewed as importance factors. Larger coefficients apply more impact on $\widetilde\Delta(\bm{x})_i$.


% \begin{figure}[t]
%     \centering
%         \centering
%         \includegraphics[width=0.8\linewidth]{fig_mnist_sensitive.eps}
%     \caption{Explanation of FNN5 for MNIST. The classification labels are 5, 8 and 9. The corresponding attack labels are 3, 3 and 1. It visualizes the normalized coefficients (VPC, VNC), and the resulting weighted images.}
%     \label{fig:mnist_sensitive}
% \end{figure}


% \paragraph{Visualization of the Coefficients for MNIST.}
% Intuitively, the larger the absolute value of the coefficient is, the more important the corresponding pixel is. There is a simple way to visualize it by normalizing each coefficient to a value in $[0,255]$.   We visualize the positive and negative coefficients separately as follows:
% \begin{itemize}
%     \item Visualizing Negative Coefficients (VNC): The column VNC shows the normalized image in which bright pixels are negative to the attack of the classification label if the value of these pixels increases.  The weighted VNC is obtained by VNC multiplied by the original image pixel wise. Its visualization intuitively shows which pixels are significantly negative to attack.%Interestingly, if  the original image is multiplied with it pixel wise, we observe a bit part of the image that is less likely useful for the attacking image. \lrj{It is still useful! but it's value will decrease not incrase} 
%     \item Visualizing Positive Coefficients (VPC): Oppositely, the column VPC shows the normalized image in which bright pixels are positive to the attack of the classification label if the value of these pixels increases. Similarly, the weighted VPC shows which pixels are significantly positive to attack.
% \end{itemize}

% In Fig.~\ref{fig:mnist_sensitive}, we illustrate the visualization for three images in MNIST. For instance, the left part of the number ``8'' is the most bright on weighted VNC, so the pixels in this part are the key features to the classification of ``8'' against ``3'', while on weighted VPC bright pixels lie mostly in the right part, and they are attempting hardest to make the original image classified as ``3''. From the aspect of human beings, this explanation is quite fantastic since the right part (weighted VPC) indeed looks like a number ``3'', and the left part (weighted VNC) makes the image no longer ``3'' in our eyes.

% \paragraph{Visualization of the Coefficients for CIFAR-10.}
% Unlike MNIST, the CIFAR-10 dataset is in color, and the brightness (the value of the pixels) does not have a close connection to the existence of the object to be recognized. Actually, the coefficients multiplied by pixel values do not provide meaningful images. 
    
% The color pixel has three channels and each channel has an independent coefficient, so each pixel has three coefficients, $(c_1,c_2,c_3)$, for each of the channels respectively. We take the $L_2$ norm and compute $(c_1^2+c_2^2+c_3^2)^\frac{1}{2}$ as a measure of the pixel. Using the measure, we mask the image by removing $20\%$, $40\%$, $60\%$, and $80\%$ of the less important pixels. Fig.~\ref{fig:netmaskcifar} shows the results on CIFAR-10. We observe that the resulting picture values the part around the head more than others. We anticipate that the horse and airplane have the same \emph{attacking preference}, as no essential differences can be observed. Interestingly, we observe masked image for ResNet152 is more scattered than VGG16.


% \begin{figure}[t]
%     \centering
%         \includegraphics[width=0.8\linewidth]{fig_exp_cifar_3.eps}
%     \caption{Explanation of VGG16 and ResNet152 for CIFAR-10. The classification label is deer. The attacking labels are airplane and horse, respectively.}
%     \label{fig:netmaskcifar}
% \end{figure}
% \fi


